Fundamental Parameters and Chemical Composition of Arcturus

We derive a self-consistent set of atmospheric parameters and abundances of 17 elements for the red giant star Arcturus: Teff = 4286+/-30 K, logg = 1.66+/-0.05, and [Fe/H] = -0.52+/-0.04. The effective temperature was determined using model atmosphere fits to the observed spectral energy distribution from the blue to the mid-infrared (0.44 to 10 um). The surface gravity was calculated using the trigonometric parallax of the star and stellar evolution models. A differential abundance analysis relative to the solar spectrum allowed us to derive iron abundances from equivalent width measurements of 37 FeI and 9 FeII lines, unblended in the spectra of both Arcturus and the Sun; the [Fe/H] value adopted is derived from FeI lines. We also determine the mass, radius, and age of Arcturus: M = 1.08+/-0.06 Msun, R = 25.4+/-0.2 Rsun, and t = 7.1(+1.5/-1.2) Gyr. Finally, abundances of the following elements are measured from an equivalent width analysis of atomic features: C, O, Na, Mg, Al, Si, K, Ca, Sc, Ti, V, Cr, Mn, Co, Ni, and Zn. We find the chemical composition of Arcturus typical of that of a local thick-disk star, consistent with its kinematics.

==> table5full.tex <==
C\,\textsc{i} & 5380.34 & 7.68 &  -1.62 &  21.3 & 8.42 & 0.01 &   9.4 & 8.35 & 0.01 & -0.07 & 0.02 \\
C\,\textsc{i} & 8335.15 & 7.68 &  -0.44 &  89.5 & 8.37 & 0.02 &  29.0 & 8.32 & 0.02 & -0.05 & 0.03 \\
C\,\textsc{i} & 9078.28 & 7.48 &  -0.57 & 106.3 & 8.47 & 0.02 &  33.1 & 8.30 & 0.02 & -0.17 & 0.03 \\
C\,\textsc{i} & 9111.80 & 7.49 &  -0.30 & 128.1 & 8.40 & 0.02 &  45.0 & 8.32 & 0.02 & -0.08 & 0.03 \\

O\,\textsc{i} & 5577.34 & 1.97 &  -8.24 & \nodata      & 8.69 & \nodata     &  10.5 & 8.68 & 0.01 & -0.01 & 0.01 \\
O\,\textsc{i} & 6300.30 & 0.00 &  -9.72 & \nodata      & 8.69 & \nodata     &  68.1 & 8.66 & 0.02 & -0.03 & 0.02 \\
O\,\textsc{i} & 6363.78 & 0.02 & -10.19 & \nodata      & 8.69 &  \nodata    &  31.1 & 8.66 & 0.01 & -0.03 & 0.01 \\

Na\,\textsc{i} & 4751.82 & 2.10 &  -2.08 &  11.5 & 6.20 & 0.01 &  29.0 & 5.77 & 0.01 & -0.43 & 0.01 \\
Na\,\textsc{i} & 5148.84 & 2.10 &  -2.04 &  12.9 & 6.21 & 0.01 &  35.5 & 5.83 & 0.01 & -0.38 & 0.02 \\
Na\,\textsc{i} & 6154.23 & 2.10 &  -1.55 &  37.0 & 6.26 & 0.01 &  73.3 & 5.84 & 0.02 & -0.42 & 0.03 \\
Na\,\textsc{i} & 6160.75 & 2.10 &  -1.25 &  55.8 & 6.25 & 0.02 &  92.9 & 5.82 & 0.03 & -0.43 & 0.03 \\

Mg\,\textsc{i} & 4730.04 & 4.34 &  -2.39 &  65.4 & 7.64 & 0.02 & 110.4 & 7.56 & 0.04 & -0.08 & 0.05 \\
Mg\,\textsc{i} & 5711.09 & 4.34 &  -1.73 & 115.8 & 7.63 & 0.02 & 156.0 & 7.55 & 0.04 & -0.08 & 0.05 \\
Mg\,\textsc{i} & 6318.72 & 5.11 &  -1.95 &  43.0 & 7.52 & 0.01 &  67.2 & 7.31 & 0.02 & -0.21 & 0.03 \\
Mg\,\textsc{i} & 6319.24 & 5.11 &  -2.32 &  25.7 & 7.59 & 0.01 &  53.4 & 7.48 & 0.02 & -0.11 & 0.02 \\
Mg\,\textsc{i} & 7657.61 & 5.11 &  -1.28 & 111.8 & 7.67 & 0.02 & 125.2 & 7.45 & 0.04 & -0.22 & 0.04 \\

Al\,\textsc{i} & 6696.02 & 3.14 &  -1.48 &  39.3 & 6.41 & 0.01 &  91.0 & 6.30 & 0.02 & -0.11 & 0.03 \\
Al\,\textsc{i} & 6698.67 & 3.14 &  -1.78 &  22.5 & 6.38 & 0.01 &  61.1 & 6.17 & 0.02 & -0.21 & 0.02 \\
Al\,\textsc{i} & 7835.31 & 4.02 &  -0.69 &  50.1 & 6.50 & 0.01 &  69.5 & 6.30 & 0.02 & -0.20 & 0.02 \\
Al\,\textsc{i} & 7836.13 & 4.02 &  -0.45 &  63.2 & 6.41 & 0.01 &  82.8 & 6.25 & 0.02 & -0.16 & 0.03 \\

Si\,\textsc{i} & 5684.48 & 4.95 &  -1.55 &  61.4 & 7.44 & 0.02 &  69.4 & 7.24 & 0.02 & -0.20 & 0.03 \\
Si\,\textsc{i} & 5690.42 & 4.93 &  -1.77 &  51.5 & 7.49 & 0.02 &  61.9 & 7.30 & 0.02 & -0.19 & 0.03 \\
Si\,\textsc{i} & 5701.10 & 4.93 &  -1.95 &  37.9 & 7.44 & 0.01 &  48.0 & 7.23 & 0.02 & -0.21 & 0.02 \\
Si\,\textsc{i} & 5772.15 & 5.08 &  -1.65 &  53.2 & 7.53 & 0.01 &  61.5 & 7.37 & 0.02 & -0.16 & 0.03 \\
Si\,\textsc{i} & 5793.07 & 4.93 &  -1.96 &  43.9 & 7.55 & 0.01 &  53.7 & 7.34 & 0.02 & -0.21 & 0.02 \\

K\,\textsc{i} & 7698.97 & 0.00 &  -0.18 & 164.0 & 5.31 & 0.02 & 253.0 & 4.99 & 0.04 & -0.32 & 0.05 \\

Ca\,\textsc{i} & 4512.27 & 2.53 &  -1.90 &  25.5 & 6.33 & 0.01 &  64.0 & 5.85 & 0.02 & -0.48 & 0.03 \\
Ca\,\textsc{i} & 5260.39 & 2.52 &  -1.72 &  33.3 & 6.30 & 0.01 &  81.9 & 5.89 & 0.03 & -0.41 & 0.03 \\
Ca\,\textsc{i} & 5867.56 & 2.93 &  -1.57 &  25.9 & 6.33 & 0.01 &  62.6 & 5.92 & 0.02 & -0.41 & 0.02 \\
Ca\,\textsc{i} & 6161.30 & 2.52 &  -1.27 &  63.2 & 6.30 & 0.02 & 112.5 & 5.87 & 0.03 & -0.43 & 0.04 \\
Ca\,\textsc{i} & 6166.44 & 2.52 &  -1.14 &  71.7 & 6.30 & 0.02 & 121.2 & 5.89 & 0.04 & -0.41 & 0.05 \\
Ca\,\textsc{i} & 6169.04 & 2.52 &  -0.80 &  98.6 & 6.34 & 0.02 & 150.0 & 6.02 & 0.04 & -0.32 & 0.05 \\
Ca\,\textsc{i} & 6169.56 & 2.53 &  -0.48 & 124.8 & 6.31 & 0.02 & 164.1 & 5.91 & 0.04 & -0.40 & 0.05 \\
Ca\,\textsc{i} & 6455.60 & 2.52 &  -1.34 &  59.0 & 6.37 & 0.02 & 115.5 & 5.97 & 0.04 & -0.40 & 0.05 \\
Ca\,\textsc{i} & 6471.66 & 2.53 &  -0.69 &  96.3 & 6.37 & 0.03 & 158.1 & 6.04 & 0.05 & -0.33 & 0.06 \\
Ca\,\textsc{i} & 6499.65 & 2.52 &  -0.82 &  91.0 & 6.42 & 0.03 & 150.7 & 6.05 & 0.05 & -0.37 & 0.05 \\

Sc\,\textsc{i} & 4743.82 & 1.45 &   2.64 &   8.3 & 2.96 & 0.01 &  78.3 & 2.69 & 0.03 & -0.28 & 0.03 \\
Sc\,\textsc{i} & 5081.56 & 1.45 &   2.94 &  10.0 & 2.99 & 0.01 &  80.0 & 2.62 & 0.03 & -0.37 & 0.04 \\
Sc\,\textsc{i} & 5484.63 & 1.85 &   1.41 &   3.2 & 3.14 & 0.01 &  34.2 & 2.72 & 0.01 & -0.43 & 0.01 \\
Sc\,\textsc{i} & 5671.83 & 1.45 &   3.13 &  14.5 & 3.11 & 0.01 & 111.1 & 3.04 & 0.04 & -0.07 & 0.04 \\

Sc\,\textsc{ii} & 5357.20 & 1.51 &  -2.11 &   5.1 & 3.14 & 0.01 &  24.9 & 2.82 & 0.01 & -0.32 & 0.02 \\
Sc\,\textsc{ii} & 5552.23 & 1.46 &  -2.28 &   4.6 & 3.20 & 0.01 &  24.5 & 2.91 & 0.01 & -0.29 & 0.01 \\
Sc\,\textsc{ii} & 5684.21 & 1.51 &  -1.07 &  36.8 & 3.19 & 0.02 &  87.9 & 2.90 & 0.03 & -0.29 & 0.03 \\
Sc\,\textsc{ii} & 6245.64 & 1.51 &  -1.04 &  35.2 & 3.09 & 0.01 &  90.0 & 2.86 & 0.03 & -0.23 & 0.04 \\
Sc\,\textsc{ii} & 6300.75 & 1.51 &  -1.95 &   6.5 & 3.06 & 0.01 &  32.9 & 2.82 & 0.01 & -0.24 & 0.02 \\
Sc\,\textsc{ii} & 6320.84 & 1.50 &  -1.92 &   8.7 & 3.16 & 0.01 &  39.7 & 2.90 & 0.01 & -0.26 & 0.02 \\
Sc\,\textsc{ii} & 6604.58 & 1.36 &  -1.31 &  36.4 & 3.22 & 0.02 &  84.8 & 2.82 & 0.03 & -0.41 & 0.03 \\

Ti\,\textsc{i} & 5219.70 & 0.02 &  -2.24 &  28.8 & 4.97 & 0.01 & 155.0 & 4.74 & 0.06 & -0.23 & 0.06 \\
Ti\,\textsc{i} & 5295.77 & 1.07 &  -1.58 &  13.0 & 4.89 & 0.01 & 104.5 & 4.58 & 0.03 & -0.32 & 0.04 \\
Ti\,\textsc{i} & 5490.15 & 1.46 &  -0.88 &  22.1 & 4.86 & 0.01 & 112.9 & 4.54 & 0.04 & -0.32 & 0.04 \\
Ti\,\textsc{i} & 5702.66 & 2.29 &  -0.59 &   8.1 & 4.85 & 0.01 &  63.0 & 4.53 & 0.02 & -0.32 & 0.02 \\
Ti\,\textsc{i} & 5716.44 & 2.30 &  -0.72 &   6.2 & 4.85 & 0.01 &  64.2 & 4.68 & 0.02 & -0.17 & 0.02 \\
Ti\,\textsc{i} & 6092.79 & 1.89 &  -1.32 &   4.1 & 4.85 & 0.01 &  58.3 & 4.61 & 0.02 & -0.24 & 0.02 \\
Ti\,\textsc{i} & 6303.75 & 1.44 &  -1.51 &   8.2 & 4.91 & 0.01 &  92.1 & 4.66 & 0.03 & -0.25 & 0.03 \\
Ti\,\textsc{i} & 6312.23 & 1.46 &  -1.50 &   8.0 & 4.90 & 0.01 &  91.7 & 4.66 & 0.03 & -0.24 & 0.03 \\
Ti\,\textsc{i} & 6599.10 & 0.90 &  -2.03 &   9.9 & 4.97 & 0.01 & 115.2 & 4.73 & 0.03 & -0.24 & 0.04 \\
Ti\,\textsc{i} & 7357.73 & 1.44 &  -1.07 &  23.1 & 4.95 & 0.01 & 131.8 & 4.69 & 0.04 & -0.27 & 0.04 \\
Ti\,\textsc{i} & 8675.37 & 1.07 &  -1.61 &  19.7 & 4.95 & 0.01 & 148.9 & 4.72 & 0.03 & -0.23 & 0.04 \\
Ti\,\textsc{i} & 8682.98 & 1.05 &  -1.88 &  12.2 & 4.96 & 0.01 & 129.5 & 4.72 & 0.03 & -0.24 & 0.04 \\
Ti\,\textsc{i} & 8734.71 & 1.05 &  -2.33 &   5.3 & 5.00 & 0.01 &  94.9 & 4.72 & 0.02 & -0.29 & 0.03 \\

Ti\,\textsc{ii} & 4583.41 & 1.17 &  -2.87 &  31.3 & 4.97 & 0.01 &  82.0 & 4.65 & 0.03 & -0.32 & 0.03 \\
Ti\,\textsc{ii} & 4708.66 & 1.24 &  -2.37 &  50.0 & 4.95 & 0.02 & 100.1 & 4.61 & 0.04 & -0.34 & 0.05 \\
Ti\,\textsc{ii} & 5336.78 & 1.58 &  -1.63 &  70.9 & 4.95 & 0.03 & 125.1 & 4.73 & 0.06 & -0.22 & 0.06 \\
Ti\,\textsc{ii} & 5418.77 & 1.58 &  -2.11 &  49.0 & 4.95 & 0.02 &  97.8 & 4.65 & 0.04 & -0.30 & 0.04 \\

V\,\textsc{i} & 6039.73 & 1.06 &  -0.65 &  12.5 & 3.90 & 0.01 & 107.2 & 3.57 & 0.03 & -0.33 & 0.04 \\
V\,\textsc{i} & 6081.44 & 1.05 &  -0.58 &  14.6 & 3.90 & 0.01 & 115.5 & 3.61 & 0.03 & -0.29 & 0.04 \\
V\,\textsc{i} & 6090.21 & 1.08 &  -0.06 &  33.3 & 3.90 & 0.01 & 138.5 & 3.53 & 0.06 & -0.37 & 0.06 \\
V\,\textsc{i} & 6119.53 & 1.06 &  -0.32 &  22.0 & 3.87 & 0.01 & 121.5 & 3.48 & 0.04 & -0.39 & 0.04 \\
V\,\textsc{i} & 6135.36 & 1.05 &  -0.75 &  10.6 & 3.90 & 0.01 & 107.1 & 3.63 & 0.04 & -0.27 & 0.04 \\
V\,\textsc{i} & 6274.65 & 0.27 &  -1.67 &   8.3 & 3.91 & 0.01 & 123.0 & 3.63 & 0.04 & -0.28 & 0.04 \\
V\,\textsc{i} & 6285.16 & 0.28 &  -4.28 &   9.9 & 3.85 & 0.01 & 128.0 & 3.57 & 0.05 & -0.28 & 0.05 \\
V\,\textsc{i} & 6531.41 & 1.22 &  -1.51 &   6.8 & 3.92 & 0.01 &  86.8 & 3.59 & 0.02 & -0.33 & 0.03 \\

Cr\,\textsc{i} & 4708.02 & 3.17 &   0.09 &  55.9 & 5.49 & 0.02 &  88.6 & 4.84 & 0.03 & -0.65 & 0.04 \\
Cr\,\textsc{i} & 4801.05 & 3.12 &  -0.13 &  49.0 & 5.58 & 0.02 &  86.2 & 4.95 & 0.03 & -0.63 & 0.04 \\
Cr\,\textsc{i} & 4936.34 & 3.11 &  -0.24 &  45.3 & 5.59 & 0.02 &  84.6 & 4.98 & 0.04 & -0.61 & 0.04 \\
Cr\,\textsc{i} & 5272.01 & 3.45 &  -0.42 &  23.9 & 5.57 & 0.01 &  51.8 & 4.99 & 0.02 & -0.58 & 0.02 \\
Cr\,\textsc{i} & 5287.20 & 3.44 &  -0.89 &  11.1 & 5.61 & 0.01 &  33.3 & 5.12 & 0.01 & -0.49 & 0.02 \\
Cr\,\textsc{i} & 5300.74 & 0.98 &  -2.08 &  58.0 & 5.58 & 0.02 & 142.8 & 4.97 & 0.06 & -0.61 & 0.06 \\
Cr\,\textsc{i} & 5304.18 & 3.46 &  -0.68 &  15.7 & 5.61 & 0.01 &  38.2 & 5.03 & 0.01 & -0.57 & 0.02 \\
Cr\,\textsc{i} & 5628.62 & 3.42 &  -0.76 &  15.1 & 5.61 & 0.01 &  37.4 & 5.03 & 0.01 & -0.59 & 0.02 \\
Cr\,\textsc{i} & 5781.16 & 3.01 &  -1.00 &  16.1 & 5.49 & 0.01 &  45.2 & 4.86 & 0.01 & -0.64 & 0.02 \\
Cr\,\textsc{i} & 6882.48 & 3.44 &  -0.38 &  33.0 & 5.65 & 0.01 &  66.5 & 5.08 & 0.02 & -0.57 & 0.02 \\
Cr\,\textsc{i} & 6883.00 & 3.44 &  -0.42 &  30.3 & 5.63 & 0.01 &  63.4 & 5.07 & 0.02 & -0.56 & 0.02 \\

Mn\,\textsc{i} & 4671.69 & 2.89 &  -1.66 &  12.8 & 5.38 & 0.01 &  40.5 & 4.66 & 0.01 & -0.71 & 0.02 \\
Mn\,\textsc{i} & 4709.71 & 2.89 &  -0.49 &  67.8 & 5.58 & 0.03 & 110.8 & 4.89 & 0.05 & -0.70 & 0.06 \\
Mn\,\textsc{i} & 4739.11 & 2.94 &  -0.60 &  60.6 & 5.56 & 0.03 & 101.2 & 4.83 & 0.04 & -0.73 & 0.05 \\
Mn\,\textsc{i} & 5004.89 & 2.92 &  -1.64 &  14.1 & 5.42 & 0.01 &  40.0 & 4.64 & 0.01 & -0.77 & 0.02 \\
Mn\,\textsc{i} & 5388.54 & 3.37 &  -1.62 &   6.0 & 5.39 & 0.01 &  17.0 & 4.70 & 0.01 & -0.70 & 0.01 \\

Co\,\textsc{i} & 5212.69 & 3.51 &  -0.11 &  21.0 & 4.86 & 0.01 &  68.4 & 4.69 & 0.02 & -0.17 & 0.03 \\
Co\,\textsc{i} & 5280.63 & 3.63 &  -0.03 &  20.3 & 4.86 & 0.01 &  58.3 & 4.57 & 0.02 & -0.29 & 0.02 \\
Co\,\textsc{i} & 5301.04 & 1.71 &  -1.94 &  21.6 & 4.95 & 0.01 & 109.0 & 4.89 & 0.06 & -0.05 & 0.06 \\
Co\,\textsc{i} & 5352.04 & 3.58 &   0.06 &  27.0 & 4.89 & 0.01 &  68.0 & 4.59 & 0.02 & -0.30 & 0.03 \\
Co\,\textsc{i} & 5647.23 & 2.28 &  -1.56 &  15.6 & 4.92 & 0.01 &  79.8 & 4.67 & 0.03 & -0.25 & 0.03 \\
Co\,\textsc{i} & 6093.14 & 1.74 &  -2.44 &  10.2 & 5.03 & 0.01 &  87.4 & 4.91 & 0.03 & -0.12 & 0.03 \\
Co\,\textsc{i} & 6455.00 & 3.63 &  -0.25 &  16.5 & 4.92 & 0.01 &  54.6 & 4.68 & 0.02 & -0.23 & 0.02 \\

Ni\,\textsc{i} & 5157.98 & 3.61 &  -1.51 &  20.0 & 6.15 & 0.01 &  41.5 & 5.68 & 0.01 & -0.48 & 0.02 \\
Ni\,\textsc{i} & 5537.11 & 3.85 &  -2.20 &   3.2 & 6.15 & 0.01 &   7.0 & 5.67 & 0.01 & -0.49 & 0.01 \\
Ni\,\textsc{i} & 6176.80 & 4.09 &  -0.26 &  65.6 & 6.11 & 0.02 &  85.3 & 5.67 & 0.03 & -0.44 & 0.04 \\
Ni\,\textsc{i} & 6204.60 & 4.09 &  -0.82 &  23.1 & 6.24 & 0.01 &  39.0 & 5.82 & 0.02 & -0.43 & 0.02 \\
Ni\,\textsc{i} & 6223.99 & 4.11 &  -1.10 &  28.4 & 6.18 & 0.01 &  43.2 & 5.71 & 0.01 & -0.47 & 0.02 \\
Ni\,\textsc{i} & 6378.26 & 4.15 &  -1.05 &  33.1 & 6.24 & 0.01 &  50.0 & 5.81 & 0.02 & -0.43 & 0.02 \\

Zn\,\textsc{i} & 4810.53 & 4.08 &  -0.16 &  78.2 & 4.57 & 0.03 &  86.2 & 4.15 & 0.04 & -0.41 & 0.05 \\
Zn\,\textsc{i} & 6362.35 & 5.80 &   0.14 &  22.5 & 4.55 & 0.01 &  14.9 & 4.26 & 0.01 & -0.29 & 0.02 \\

